DB-BERT: a Database Tuning Tool that "Reads the Manual"

DB-BERT is a database tuning tool that exploits information gained via natural language analysis of manuals and other relevant text documents. It uses text to identify database system parameters to tune as well as recommended parameter values. DB-BERT applies large, pre-trained language models (specifically, the BERT model) for text analysis. During an initial training phase, it fine-tunes model weights in order to translate natural language hints into recommended settings. At run time, DB-BERT learns to aggregate, adapt, and prioritize hints to achieve optimal performance for a specific database system and benchmark. Both phases are iterative and use reinforcement learning to guide the selection of tuning settings to evaluate (penalizing settings that the database system rejects while rewarding settings that improve performance). In our experiments, we leverage hundreds of text documents about database tuning as input for DB-BERT. We compare DB-BERT against various baselines, considering different benchmarks (TPC-C and TPC-H), metrics (throughput and run time), as well as database systems (Postgres and MySQL). In all cases, DB-BERT finds the best parameter settings among all compared methods. The code of DB-BERT is available online at https://itrummer.github.io/dbbert/.

==> sections/replies.tex <==
\newcommand\rev[1]{{\color{red}#1}}

\theoremstyle{plain}
\newtheorem{question}{Question}
\theoremstyle{definition}
\newtheorem{answer}{Answer}

\section*{Overview of Changes in Revision}

\newcommand{\stab}{\vspace{1.2ex}\noindent}

\vspace{0.25cm}

Dear shepherd, dear reviewers and editor,

\vspace{0.25cm}

We thank all reviewers for their insightful comments! We have addressed all changes requested in the meta-review as well as  other points raised by the reviewers. Below, we outline how we addressed the suggestions for each of the reviews. We also marked the most important changes in the revised paper in red.

\subsection*{Meta-Review}

\begin{question}
Required changes: Please address O3 and O4 from Reviewer \#2.
\end{question}
\begin{answer}
We addressed both points as outlined in more detail below (section on Reviewer \#2 review).
\end{answer}

\subsection*{Reviewer 1}

\begin{question}
O1: This work can be viewed as a special case of semantic parsing and reinforcement learning. The similar techniques have been extensively studied in the area of seq2sql where a piece of text is translated to a SQL statement. Similarly, one can examine whether the mapped SQL statement can be successfully executed or not. The run time feedback in this work is more straightforward. The authors might consider reading/referring new progress in that domain and further improve the NLP part of DB-BERT.
\end{question}

\begin{answer}
We added a new subsection (Section~\ref{sub:nlqi}) to our related work section, discussing prior work on text-to-SQL translation.
\end{answer}

\subsection*{Reviewer 2}

\begin{question}
O1. First of all, the scope of the parameters being tuned is not clarified upfront in the paper. The paper claims that DB-BERT finds best parameter settings among all competing methods. Based on the examples and discussions it seems like only parameters with numeric and boolean values that are related to RAM, hard disk, and CPU cores are considered. What would be an appropriate characterization of the types of parameters that DB-BERT currently supports? How will DB-BERT handle parameters like fsync (on/off) in Postgres based on reading the manual? Setting “fsync=off” will improve performance at the risk of losing data.

O2. A discussion on how DB-BERT can be extended to support various parameter settings and objectives that cannot currently be supported is required (for example, fsync in postgres). The characterizations in O1 coupled with a discussion on possible extensions will help readers better understand the strengths and limitations of the system.

... Thanks for the response. The authors' response to O1 and O2 (scope and extensions) were satisfactory. A discussion on both of these aspects in a revision should suffice (the authors can make the related work discussion more concise to make space).
\end{question}

\begin{answer}
We added a clarification on parameter scope (O1), following our reply in the author response, at the beginning of Section~\ref{sec:overview} (end of second paragraph).

We expanded our conclusion section (Section~\ref{sec:conclusion}) by detailing extensions to more complex tuning objectives (focusing, in particular, on objectives referenced in our prior author response).
\end{answer}

% Why is “15 minute tuning time frame” a consideration for the problem (time was not mentioned as a constraint in definition 3.2)? DB-BERT also has the additional overhead of hint extraction and ordering. Therefore, the authors should explore the impact of using the recommended number of iterations on the execution performance of DDPG+.

%While the authors mention that DB-BERT considers more parameters which would significantly increase the runtime for the DDPG++ baseline [27], running only seven or eight iterations as opposed to 150 as in [27] is a drastic decrease. Therefore, the comparison doesn't seem fair. I agree that taking less time to tune is beneficial. However, it doesn't paint the whole picture --- what is the throughput of DDPG++ when it is run for more iterations.

\begin{question}
O3. In Section 8.4, the choice of allowing only a few iterations for DDPG+ was not well motivated. ...

However, the choice of limiting to the number of iterations of the DDPG++ baseline (response to O3) is not well-motivated. ... I suggest the authors conduct either of the following two experiments to showcase DB-BERT's effectiveness:

a) ...
or,
b) keep using DDPG++ [27] as a baseline but run for a reasonable number of iterations and then report the results. One approach can be to set tuning time to 25 minutes (as previous approaches like DDPG [33]) as a justification for using a time-constraint. The choice of 15 minutes if not well justified.

%use DDPG [33] as a baseline which considers a higher number of knobs and has a online tuning time of 25 minutes (DDPG++[27] claims to improve over DDPG [33] but for only 10 knobs. DDPG [33] considers 266 knobs)

Running either (a) or (b) should suffice.
\end{question}

\begin{answer}
We chose option (b) and re-ran all experiments with a tuning time of 25 minutes, as suggested by the reviewer.
\end{answer}

\begin{question}
O4. How were the values for multiplication M and weights W chosen?
...
Also, the authors didn't respond to my O4 (rationale behind the choice of parameter values). Futher clarification will help replicate DB-BERT for other DMBSs.
\end{question}

\begin{answer}
DB-BERT uses reinforcement learning to pick the appropriate multiplicator and weight for each specific hint from a pre-defined set of alternative values. We consider the set $\{1/4,1/2,1,2,4\}$ as alternative values for the multiplicator and the set $\{0,2,4,8,16\}$ as alternative values for the weight. We use the same set of alternative values for all our experiments in the paper.

In both cases, we use five alternative values. We want to avoid choosing more values than necessary since it increases the size of the search space for reinforcement learning (thereby, potentially, increasing convergence time). Furthermore, the reinforcement learning frameworks we use (OpenAI gym) makes it easy to model environments in which the same number of actions is available in each state. Since we have five actions to choose the hint type (no hint, absolute value, relative to RAM size, relative to disk size, relative to the number of cores), it is convenient to have the same number of actions to choose weight and multiplicator. 

For the multiplicator, we consider a set of values that allows DB-BERT to slightly correct values given in text (which may not be optimal for each workload). If values given in text are off by more than factor four, it seems more reasonable to disregards the associated hint altogether. This can be done by setting a weight of zero. The other weights allow increasing the relative importance of specific hints. The lowest (non-zero) weight differs from the highest one by factor 8. This means that a single hint cannot receive more weight than 8 other hints combined (which seems reasonable). 

%We did not experiment with different values for the alternative values for weights and multiplicators. We cannot exclude that other values work slightly better. However, we doubt that significant improvements can be achieved.

In the revised paper, we elaborate on the selection of values for weights and multiplicators in Section~\ref{sub:setup}.
\end{answer}

\subsection*{Reviewer 3}

\begin{question}
O1. Exposition can be improved to clarify what is manually provided and what is automatically extracted for hint generation.
\end{question}

\begin{answer}
We clarified at the end of the introduction which parts of DB-BERT's inputs are manually provided, in comparison to manual overheads of a prior approach for NLP-enhanced database tuning.
\end{answer}

\begin{question}
O2. The approach at times comes across as overly convoluted and piecemeal, lacking conceptual clarity and coherence. In addition to O1, maybe a figure showing the end-to-end pipeline early in the paper can help the reader.
\end{question}

\begin{answer}
We changed Figure~\ref{fig:overview} to illustrate the end-to-end pipeline in much more detail. We also rewrote the associated text description to describe all steps in the pipeline and their interplay. Thank you for the suggestion!
\end{answer}

\begin{question}
M1. Charts are too crowded. Consider revising them for improved readability (e.g., increase chart area sizes, reduce marker symbol sizes, remove redundant markers \& just use color for categories, etc.)
\end{question}

\begin{answer}
We revised the plots by removing markers (e.g., Figure~\ref{fig:docanalysis}), or reducing marker sizes (e.g., reduced size of X markers in Figure~\ref{fig:ddpgTpch}).
\end{answer}

\begin{question}
M2. “with exploration (exploiting” --> “with exploitation (exploiting”
\end{question}

\begin{answer}
We fixed the typo, changing exploration to exploitation.
\end{answer}

\begin{question}
M3. Matter of style but consider removing the specifiers “Google’s” and “Google’s famous” before “BERT.” They sound a bit too colloquial.
\end{question}

\begin{answer}
We removed these specifiers.
\end{answer}
